Modified Gravity and Dark Energy models Beyond $w(z)$CDM Testable by LSST

One of the main science goals of the Large Synoptic Survey Telescope (LSST) is to uncover the nature of cosmic acceleration. In the base analysis, possible deviations from the Lambda-Cold-Dark-Matter ($\Lambda$CDM) background evolution will be probed by fitting a $w(z)$CDM model, which allows for a redshift-dependent dark energy equation of state with $w(z)$, within general relativity (GR). A rich array of other phenomena can arise due to deviations from the standard $\Lambda$CDM+GR model though, including modifications to the growth rate of structure and lensing, and novel screening effects on non-linear scales. Concrete physical models are needed to provide consistent predictions for these (potentially small) effects, to give us the best chance of detecting them and separating them from astrophysical systematics. A complex plethora of possible models has been constructed over the past few decades, with none emerging as a particular favorite. This document prioritizes a subset of these models along with rationales for further study and inclusion into the LSST Dark Energy Science Collaboration (DESC) data analysis pipelines, based on their observational viability, theoretical plausibility, and level of theoretical development. We provide references and theoretical expressions to aid the integration of these models into DESC software and simulations, and give justifications for why other models were not prioritized. While DESC efforts are free to pursue other models, we provide here guidelines on which theories appear to have higher priority for collaboration efforts due to their perceived promise and greater instructional value.

==> authors.tex <==
% Author list file generated with: mkauthlist 1.2.4 
% mkauthlist -j tex -f -c LSST Dark Energy Science Collaboration --cntrb contributions.tex authors.csv authors.tex 

\author{Mustapha Ishak}
\affiliation{Department of Physics, The University of Texas at Dallas, Richardson, TX 75083, USA}
\author{Tessa Baker}
\affiliation{Department of Physics, University of Oxford, Keble Road, Oxford OX1 3RH, UK}
\affiliation{School of Physics \& Astronomy, Queen Mary University of London, 327 Mile End Road, London E1 4NS, UK}
\author{Philip Bull}
\affiliation{School of Physics \& Astronomy, Queen Mary University of London, 327 Mile End Road, London E1 4NS, UK}
\affiliation{Radio Astronomy Laboratory, University of California Berkeley, Berkeley, CA 94720, USA}
\author{Eske M. Pedersen}
\affiliation{Department of Physics, The University of Texas at Dallas, Richardson, TX 75083, USA}
\author{Jonathan Blazek}
\affiliation{Center for Cosmology and Astroparticle Physics, Ohio State, Columbus, OH 43210, USA}
\affiliation{Laboratory of Astrophysics, \'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland}
\author{Pedro G. Ferreira}
\affiliation{Department of Physics, University of Oxford, Keble Road, Oxford OX1 3RH, UK}
\author{C. Danielle Leonard}
\affiliation{McWilliams Center for Cosmology, Department of Physics, Carnegie Mellon University}
\author{Weikang Lin}
\affiliation{Department of Physics, The University of Texas at Dallas, Richardson, TX 75083, USA}
\author{Eric Linder}
\affiliation{Berkeley Lab and University of California, Berkeley CA 94720 USA}
\author{Kris Pardo}
\affiliation{Department of Astrophysical Sciences, Princeton University, Princeton, NJ 08544, USA}
\author{Georgios Valogiannis}
\affiliation{Department of Astronomy, Cornell University, Ithaca, NY 14853, USA}


\collaboration{(LSST Dark Energy Science Collaboration)}


==> contributions.tex <==
Author contributions are listed below. \\
Mustapha Ishak: Co-initiated and co-led the effort and writing of this note. Coordinated and contributed to work on assessing and ranking models. Contributed to a thorough compilation of MG literature and the writing of precursory text and tables on DESC confluence page that were used for this note. Wrote most of section 2.3 on Non-local Gravity and section 4 on Systematics; Contributed to writing sections 1.1 and 1.2; Edited and reviewed all the document. \\
Tessa Baker: Wrote the Horndeski and bigravity sections (together with P.Bull and P.Ferreira) sections 4.1 and 4.2. Edited and reviewed much of the document. Collated the mathematics and derived quasistatic limits for Horndeski equations. Determined rankings of priority models according to the scheme of section 4. \\
Philip Bull: Coordinated initial work on assessing models; helped coordinate rest of project; initial writing and organization of document; general editing. \\
Eske M. Pedersen: Wrote stuff for Sections 2.4 and 2.5  addressed related comments and edited both of these sections as well \\
Jonathan Blazek: Coordination and planning for document and model selection; wrote text on systematic effects; general editing. \\
Pedro G. Ferreira: Wrote stuff. \\
C. Danielle Leonard: Wrote text. Reviewed text. Particpated in discussions. \\
Weikang Lin: Wrote stuff. \\
Eric Linder: Initial ranking formalism; detailed discussions; thorough editing.. \\
Kris Pardo: Wrote sentences and edited Sections 2.1 and Appendix A \\
Georgios Valogiannis: Wrote stuff. \\

